Out of Distribution Reasoning by Weakly-Supervised Disentangled Logic Variational Autoencoder

Out-of-distribution (OOD) detection, i.e., finding test samples derived from a different distribution than the training set, as well as reasoning about such samples (OOD reasoning), are necessary to ensure the safety of results generated by machine learning models. Recently there have been promising results for OOD detection in the latent space of variational autoencoders (VAEs). However, without disentanglement, VAEs cannot perform OOD reasoning. Disentanglement ensures a one- to-many mapping between generative factors of OOD (e.g., rain in image data) and the latent variables to which they are encoded. Although previous literature has focused on weakly-supervised disentanglement on simple datasets with known and independent generative factors. In practice, achieving full disentanglement through weak supervision is impossible for complex datasets, such as Carla, with unknown and abstract generative factors. As a result, we propose an OOD reasoning framework that learns a partially disentangled VAE to reason about complex datasets. Our framework consists of three steps: partitioning data based on observed generative factors, training a VAE as a logic tensor network that satisfies disentanglement rules, and run-time OOD reasoning. We evaluate our approach on the Carla dataset and compare the results against three state-of-the-art methods. We found that our framework outperformed these methods in terms of disentanglement and end-to-end OOD reasoning.

==> Figurefiles/FigAUROC.tex <==
\begin{figure*}
\begin{minipage}[t]{\columnwidth}% 1st minipage
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/Auroc_rain.png}
    \caption{Auroc for rain factor}
        \label{fig:WDLVAErain}

\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/Auroc_city.png}
    \caption{Auroc for city factor}
    \label{fig:WDLVAEcity}
\end{subfigure}
\caption{Auroc curves for each OOD reasoner}
\label{fig:AUROC}

\end{minipage}%
\hfill

\end{figure*}

==> Figurefiles/FigAUROC2.tex <==
\begin{figure*}
\begin{multicols}{2}
   \includegraphics[width=0.5\linewidth]{newfig/Auroc_rain.png}\par 
    \includegraphics[width=0.5\linewidth]{newfig/Auroc_city.png}\par 
    \end{multicols}

\end{figure*}

==> Figurefiles/FigAUROCCity.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{newfig/Auroc_city.png}
    \caption{Auroc curve for city}
    \label{fig:overview}
\end{figure}

==> Figurefiles/FigAUROCRain.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{newfig/Auroc_rain.png}
    \caption{Auroc curve for rain}
    \label{fig:overview}
\end{figure}

==> Figurefiles/Figurelat.tex <==
\begin{figure*}
\begin{minipage}[t]{\columnwidth}% 1st minipage
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/WDrlat3.png}
    \caption{$L_{f_{rain}}$ of WDLVAE}
        \label{fig:WDLVAErain}

\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/WDclat6.png}
    \caption{$L_{f_{city}}$ of WDLVAE}
    \label{fig:WDLVAEcity}

\end{subfigure}
%\caption{The distribution of score}
\end{minipage}%
\hfill

\begin{minipage}[t]{\columnwidth}% 1st minipage
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/JorVAErain.png}
    \caption{$L_{f{rain}}$ of HPVAE}
        \label{fig:HPVAErain}

\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/jorVAEcity.png}
    \caption{$L_{f_{city}}$ of HPVAE}
        \label{fig:HPVAEcity}

\end{subfigure}
\end{minipage}%

\hfill

\begin{minipage}[t]{\columnwidth}% 1st minipage
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/weak_rain_latent_15.png}
    \caption{$L_{f_{rain}}$ of AVVAE}
    \label{fig:AVVAErain}

\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/weak-city_latent_50.png}
    \caption{$L_{f_{city}}$ AVVAE}
    \label{fig:AVVAEcity}

\end{subfigure}
\end{minipage}%

\hfill

\begin{minipage}[t]{\columnwidth}% 1st minipage
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/pair_rain_latent_0.png}
    \caption{$L_{f_{rain}}$ of PVAE}
        \label{fig:PVAErain}

\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\linewidth}%
    \includegraphics[width=\linewidth]{newfig/pair-city_latent_0.png}
    \caption{$L_{f_{city}}$ of PVAE}
        \label{fig:PVAEcity}

\end{subfigure}
\caption{Visualization of dimensions that are used as OOD reasoner}
\label{fig:Latents}
\end{minipage}%

\end{figure*}

==> Figurefiles/Figurelat2.tex <==
\begin{figure*}
\begin{multicols}{2}
    \includegraphics[width=0.55\linewidth]{newfig/WDrlat3.png}
    \includegraphics[width=0.55\linewidth]{newfig/WDclat6.png}
    \caption{WDLVAE latent reasoers}
    \label{fig:WDLVAE}
     \includegraphics[width=0.55\linewidth]{newfig/JorVAErain.png}
    \includegraphics[width=0.55\linewidth]{newfig/jorVAEcity.png}
    \caption{HPVAE latent reasoners}
    \label{fig:HPVAE}
    \end{multicols}
\begin{multicols}{2}
   \includegraphics[width=0.55\linewidth]{newfig/weak_rain_latent_15.png}
   \includegraphics[width=0.55\linewidth]{newfig/weak-city_latent_50.png}
   \caption{AVVAE latent reasoners}
    \label{fig:AVVAE}
   \includegraphics[width=0.55\linewidth]{newfig/pair_rain_latent_0.png}
   \includegraphics[width=0.55\linewidth]{newfig/pair-city_latent_0.png}
  \caption{PVAE latent reasoners}
\label{fig:PVAE}
\end{multicols}
\centering
\begin{multicols}{2}
   \includegraphics[width=0.8\linewidth]{newfig/Auroc_rain.png}
    \includegraphics[width=0.8\linewidth]{newfig/Auroc_city.png}
    \end{multicols}
\caption{Auroc curves for rain and city reasoners}
\label{fig:AUROC}
\end{figure*}


==> Tables/MIG.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{factor}       & \textbf{Approach} & \textbf{$L_m$} & \textbf{$M_m$} & \textbf{$L_{sm}$} & \textbf{$M_{sm}$} & \textbf{MIG}  & \textbf{$E_L$} \\ \hline
\multirow{4}{*}{Rain} & $WDLVAE$          & \textbf{3}  & 0.36         & 21           & 0.01         & \textbf{0.51} & \textbf{3}  \\ \cline{2-8} 
                      & $HPVAE$         & 125         & 0.284        & 49           & 0.28         & 0.006         & 125         \\ \cline{2-8} 
                      & $AVVAE_{rain}$   & 28          & 0.008        & 30           & 0.006        & 0.003         & 15           \\ \cline{2-8} 
                      & $PVAE_{rain}$      & 0           & 0.017        & 116          & 0.009        & 0.01          & 0           \\ \hline
\multirow{4}{*}{City} & $WDLVAE$          & \textbf{6}  & 0.69         & 3            & 0.015        & \textbf{0.98} & 6           \\ \cline{2-8} 
                      & $HPVAE$         & 49          & 0.156        & 125          & 0.151        & 0.007         & 125         \\ \cline{2-8} 
                      & $AVVAE_{city}$   & 94          & 0.008        & 93           & 0.005        & 0.004         & 50           \\ \cline{2-8} 
                      & $PVAE_{city}$     & 0           & 0.69         & 15           & 0.375        & 0.45          & 0           \\ \hline
\end{tabular}
\caption{Expected dimension $E_L$, most informative ($L_m$) and second most informative ($L_{sm}$) latent variable and their mutual information gain $M_m$ and $M_{sm}$}
\label{tab:MIG}
\end{table}

==> Tables/Symbols.tex <==
\begin{table}[]
%\centering
\begin{center}
    
\begin{tabular}{|c|c|c|}
\hline
\textbf{Symbol}       & \textbf{definition}                   & \textbf{Description}                 \\ \hline 
$\sim: N(a)$          & 1-a                                   & standard negation                    \\ \hline
$\wedge: T(a,b)$      & $a.b=\sum{x_iy_i}$ & Product t-Norm. \\ & & (.) is inner \\ && product \\ \hline
$\vee:S(a,b)$         & a+b-a.b                               & Dual t-conorm                        \\ \hline
$\rightarrow: I(a,b)$ & 1-a+a.b                               & Reichenbach \\ & & implication              \\ \hline

$\forall$ : $A_{pME}(a_1,..,a_{n})$ & $1-\sqrt{(\frac{1}{n} \sum_{i=1}^{|n|}(1-a_i)^2)}$  & Generalized \\ && mean \\& & w.r.t. the error \\ \hline

$\exists:A_{pM}(a1,..,a_{n})$ & $\sqrt{(\frac{1}{n} \sum_{i=1}^{|n|}a_i^2)}$ &  Generalized \\&& mean  \\ \hline
\end{tabular}
\caption{Real logic fuzzy operation and their definition}
\label{tab:Reallog}

\end{center}

\end{table}
